Predicting Parking Lot Availability by Graph-to-Sequence Model: A Case Study with SmartSantander

Nowadays, so as to improve services and urban areas livability, multiple smart city initiatives are being carried out throughout the world. SmartSantander is a smart city project in Santander, Spain, which has relied on wireless sensor network technologies to deploy heterogeneous sensors within the city to measure multiple parameters, including outdoor parking information. In this paper, we study the prediction of parking lot availability using historical data from more than 300 outdoor parking sensors with SmartSantander. We design a graph-to-sequence model to capture the periodical fluctuation and geographical proximity of parking lots. For developing and evaluating our model, we use a 3-year dataset of parking lot availability in the city of Santander. Our model achieves a high accuracy compared with existing sequence-to-sequence models, which is accurate enough to provide a parking information service in the city. We apply our model to a smartphone application to be widely used by citizens and tourists.

==> algorithms/learning.tex <==

% モデルの学習アルゴリズム
\begin{algorithm}[!t]
    \caption{Learning algorithm} \label{train:algorithm}
        \DontPrintSemicolon
            \SetKwInOut{Input}{input}
    	    \SetKwInOut{Output}{output}
    	    \SetKwInOut{Parameter}{parameter}
    	    \Input{Dataset $\mathcal{D}$, workload $W$, the number of computers $M$, demo data $B_\mathit{d}$, demo partitions $\mathcal{P}_d$}
    	    \Parameter{Update weight frequency $U$, demo ratio $\rho$, the number of episodes $e_{max}$}
    	    \Output{Best partitions $\mathcal{P}_b$}
    	    {\bf procedure} {\sc Pre-training}\\
    	    Initialize the main network $\theta$ and target network $\theta'$\;
            $B_\mathit{demo} \gets B_\mathit{d}$\;
            
            \For{$e=1, \ldots, e_{max}$}{
                Sample mini-batch $B$ from $B_\mathit{demo}$\;
                Train main network $\theta$ with $B$\;
                {\bf if} $(e \bmod U) = 0$ {\bf then} $\theta' \leftarrow \theta$\;
                Generate partitions $\mathcal{P}_e$ by agent actions\;
                {\bf if} $\mathcal{P}_e= \mathcal{P}_d$  {\bf then} {\bf break}
            }
            
            {\bf procedure} {\sc Main-training}\\
            $\mathit{step} \gets 0$, $\mathcal{P}_b \gets \mathcal{P}_d$, $B_\mathit{agent} \gets \varnothing$\;
            \For{$e=1, \ldots, e_{max}$}{
                Reset state $s_0$, $B_\mathit{tmp} \gets \varnothing$\;
                \For{$t=1, \ldots, M-1$}{
                    Choose action $a_t$ with our $\epsilon$-greedy method by $\theta$\;
                    Execute action $a_t$ and observe state $s_{t}$\;
                    \eIf{$t \neq M-1$}{
                        $B_\mathit{tmp} \gets B_\mathit{tmp} \cup \{(s_t, a_t, 0, s_{t+n})\}$\;
                    }
                    {
                        Distribute partitions $\mathcal{P}_e$ to computers\;
                        Run operators in $W$\;
                        $r_t = (\sum_{w_i \in W}{f_i}\cdot\frac{C(\mathcal{P}_b,w_i)}{C(\mathcal{P}_e,w_i)})^2$\;
                        $B_\mathit{tmp} \gets B_\mathit{tmp} \cup \{(s_t, a_t, r_t, s_{t+n})\}$\;
                        \eIf{$r > 1$}{
                            $B_\mathit{demo} \gets B_\mathit{demo} \cup B_\mathit{tmp}$\;
                            $\mathcal{P}_b \gets \mathcal{P}_e$\;
                        }{
                            $B_\mathit{agent} \gets B_\mathit{agent} \cup B_\mathit{tmp}$
                        }
                    }
                    Sample mini-batch $B$ from $B_\mathit{demo}$ and $B_\mathit{agent}$\;
                    Train main network $\theta$ with $B$\;
                    $\mathit{step} \gets \mathit{step}+1$\;
                    {\bf if} $(\mathit{step} \bmod U) = 0$ {\bf then} $\theta' \leftarrow \theta$
                }
            }
            %{\bf end procedure}
\end{algorithm}

